LLM4Causal: Democratized Causal Tools for Everyone via Large Language Model

Large Language Models (LLMs) have shown their success in language understanding and reasoning on general topics. However, their capability to perform inference based on user-specified structured data and knowledge in corpus-rare concepts, such as causal decision-making is still limited. In this work, we explore the possibility of fine-tuning an open-sourced LLM into LLM4Causal, which can identify the causal task, execute a corresponding function, and interpret its numerical results based on users' queries and the provided dataset. Meanwhile, we propose a data generation process for more controllable GPT prompting and present two instruction-tuning datasets: (1) Causal-Retrieval-Bench for causal problem identification and input parameter extraction for causal function calling and (2) Causal-Interpret-Bench for in-context causal interpretation. By conducting end-to-end evaluations and two ablation studies, we showed that LLM4Causal can deliver end-to-end solutions for causal problems and provide easy-to-understand answers, which significantly outperforms the baselines.

==> 0_0_Internal_Knowledge_Papers_Longversion.tex <==
To explore LLMs' potential for causal decision-making processes, recent studies are majorly based on LLM's knowledge saved internally in its parameters. For example, \cite{kasneci2023chatgpt} utilizes LLM to recover pairwise causal relationships based on the metadata of the variables, instead of the data values. \cite{long2023can} further extends the approach to obtain causal graph estimates by querying LLM about the variable pairs. However, this line of approach has some limitations: First, this approach is limited to causal structure learning and cannot be applied to other causal tasks such as causal effect estimation and causal policy learning. Second, this type of approach is heavily based on internal knowledge in the LLM training corpus, which can be incomplete and outdated. Third, this approach lacks step-by-step reasoning and provides the results in a black-box way.

==> 0_1_Data_and_Tool_Usage_Papers_Longversion.tex <==
A natural candidate to overcome the above limitations is to ask the LLM to complete the causal tasks utilizing data input. %This data-enhanced LLM model could be applicable to causal structure learning, causal effect learning and policy learning. It could expand human knowledge with external data sources and also provide step-by-step reasoning for better model transparency. 
Two notable examples of such data-enhanced LLMs include i) the Advanced Data Analysis plugin of ChatGPT \citep{gpt_dap}, formerly known as the Code Interpreter \citep{codeinterpretor}, which allows users to instruct the LLM through prompts to conduct technical data analysis on self-uploaded datasets; and ii) the latest GPT-3.5/GPT-4 models that include the function calling feature \citep{gpt_function}, allowing users to introduce new functions for LLM to select from, by providing detailed descriptions and structured information about the function. Additionally, many other recent developments like ToolLLM\citep{toolllm} and GPT4Tools\citep{gpt4tools} also enable LLMs to use external tools to conduct data analysis but are not specifically tailored for the causal tasks. 

Despite their ability to analyze external datasets, all of the aforementioned data-enhanced LLMs have the following two limitations in dealing with causal problems: First, in-depth domain knowledge is required to validate the results provided by the current GPT-based models. While these models can provide a wealth of information related to the user's query, they frequently hallucinate and mislead the user with irrelevant context. For example, they may provide correlation analysis results when causal effect analysis is expected, as shown in Figure \ref{fig:interaction_1}. Second, while some existing approaches may provide guidance for implementing some classical causal methods and suggest the corresponding code script, they fail to provide end-to-end result delivery and easy-to-understand interpretation. Third, pre-trained on massive text corpus, it only provides executions for major methods contained in the training data and requires users' effort for implementing newly-released approaches as shown in Figure \ref{fig:interaction_2}. 

\begin{figure}[h]
\begin{subfigure}{0.5\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{Fig/interaction_1.png}
  \caption{User queries on causal relationships.}
  \label{fig:interaction_1}
\end{subfigure}%
\hfill
\begin{subfigure}{0.5\columnwidth}
  \centering
  \includegraphics[width=\columnwidth]{Fig/interaction_2.png}
    \caption{User queries on implementing LinGAM method. 
    }    
    \label{fig:interaction_2}
\end{subfigure}
\caption[Caption]{User interaction with ChatGPT on causal related questions.\protect\footnotemark}
\label{figure}
\end{figure}
\footnotetext{The chat histories could be found in \href{https://chat.openai.com/share/73982d06-530e-499c-9348-682dcadbcd4e}{link 1}, and \href{https://chat.openai.com/share/1134f5d4-cc78-4e31-9865-afbe28461556}{link 2}.}

==> 0_2_Structure_of_Paper_Longversion.tex <==
The rest of the paper is organized as follows. We first introduce the related work in Section \ref{Sec:related_work} and provide the problem formulation in Section \ref{Sec:problem_formulation}. In Section \ref{Sec:proposed_method}, we describe the proposed \textbf{LLM4Causal} framework in detail, and the effectiveness of the proposed method is evaluated through extensive experiments in Section \ref{Sec:experiments}. Finally, we conclude and discuss some potential future works in Section \ref{Sec:conclusion}.

==> 1_3_Shortversion_Causal_Decision_Making.tex <==
\subsection{Causal decision making}
The decision-making process, crucial in diverse real-life contexts, fundamentally relies on understanding counterfactual scenarios, thereby emphasizing the significance of causal analysis in decision-making. Recently, \citet{CDM} proposed a comprehensive framework known as Causal Decision Making \citep[CausalDM,][]{CDM}, which examines various decision-making stages through a causal lens and establishes connections among the relevant literature under the same conceptual umbrella. In general, the body of current literature can be classified into three basic categories: i) causal structure learning (CSL) \citep{spirtes2000causation, glymour2019review}
% \citep{spirtes2000causation, shimizu2006linear, zheng2018dags, yu2019dag, glymour2019review}
, which focuses on unraveling the complex causal relationships among variables, is pivotal for pinpointing vital factors that influence outcomes, either directly or indirectly; ii) causal effect learning (CEL) \citep{yao2021survey,hicks2011causal}, which is primarily concerned with quantifying the effects resulting from different causal paths within a known causal structure, typically concentrating on measuring the difference between outcomes of receiving versus not receiving treatments; and iii) causal policy learning (CPL), which involves evaluating various treatment strategies and developing optimal action plans, frequently investigated as dynamic treatment regime problems \citep{chakraborty2014dynamic} or conceptualized within the framework of reinforcement learning \citep{sutton2018reinforcement,zeng2023survey}. 

==> 1_4_Shortversion_Large_Language_Models_with_Causal_Capabilities.tex <==
\subsection{Large Language Models with Causal Capabilities}
The rapid development of LLMs has inspired some innovative methods on applying LLMs on causal graph discovery tasks. Both \citet{kiciman2023causal} and \citet{long2023can} propose to obtain the causal relationships between variables by directly querying GPT models using the variables names, assuming that LLMs can extract internal causal knowledge of those variables from the large corpus it was trained on.
% \citet{kiciman2023causal} is one of the pioneering works in this field, introducing a method that relies solely on "meta-data" (variable names) instead of specific observed variable values. Using LLMs like GPT-3.5 and GPT-4, this approach detects causal relationships between variable pairs through direct querying. Similarly, \citet{long2023can} use GPT-3 to discover causal relationships from variable names within the medical domain, motivated by the capacity of LLM to extract knowledge from the medical texts on which it was trained. 
% However, as \citet{long2023can} highlighted, the efficacy of this type of approach relies heavily on the prompts used for LLM queries and the initial training corpus of the LLM. 
In a further development, \citet{ban2023query} proposes to integrate the causal relations retrieved directly from LLMs and traditional score-based causal discovery methods. In their framework, the LLM's internal causal knowledge are utilized to guide the optimization process of score-based methods as soft or hard constraints, enhancing the performance compared to using either LLMs or traditional methods alone. \citet{gupta2023learned}, on the other hand, apply LLMs in selecting the best candidate causal discovery methods for a specific dataset rather than directly discovering the causal relations on the dataset given. 
% Their framework is claimed to be able to select the causal discovery method with the best F1 score out of a fixed set of candidates. 
Furthermore, \citet{zhang2023understanding} discusses the strengths and limitations of LLMs for causal discovery. Although LLMs have advantages in detecting causal relationships within the scope of their training data, their performance suffers when confronted with unfamiliar domains. It is worth mentioning that our approach differs from the previously mentioned studies, as none of them introduces a mechanism to automatically invoke data-based causal discovery methods, nor do they have a mechanism to translate the output into natural languages that general audiences can understand. 


==> 3_1_STEP1.tex <==

\subsection{STEP1. Interpret User Request}
\label{sec:step1}
The purpose of the first step is to translate user questions %into a causal task classification and a list of related information 
through two integrated substeps: i) problem classification and ii) attribute extraction. Initially, problem classification categorizes the input question into one of the five supported causal tasks (CGL, ATE, HTE, MA, or OPO) by inferring the underlying user intention. Following this, attribute extraction, conditioned on the task classification, extracts attribute values that are necessary for the expert tools to address the causal problem. Instead of formulating it as a sequential process, we propose to merge them into one sequence-to-sequence (seq2seq) procedure where the output is a structured JSON with the "causal\_problem" key and other task-specific keys, e.g. "dataset" ($\mathcal{D}$), "treatment" ($\mathcal{A}$), "outcome" ($\mathcal{Y}$).%, as keys for the corresponding task. 
To keep the sequential nature of the problem, we always keep the "causal\_problem" key in the first place. The required keys for each causal task are learned implicitly by the parameters of LLM. Some simulated input queries with the corresponding JSON output are shown in Table \ref{tab:input-output-example}.

\input{Tables/Table2}

% Details
Using the example of CGL task in Table \ref{tab:input-output-example} as an illustration, the output JSON has two task-specific keys conditioned on its inferred classification as a CGL task: "dataset" with the value "disaster\_risk\_reduction.csv," and "nodes", which includes 'building\_code\_compliance\_rate' and 'disaster\_preparedness\_campaigns'.%, i.e., Causal Graph Learning (CGL), which is the first object to be inferred.%and may not be directly mentioned in the input query. 
%Meanwhile, explicit references to key values are required for the remaining keys, such as "disaster\_risk\_reduction.csv" for the "dataset" key and ['building\_code\_compliance\_rate', 'disaster\_preparedness\_campaigns'] for the "nodes" key.

% Using fine-tuned LLM
Even with careful prompt engineering, it is challenging to directly adopt a pre-trained LLM for such a seq2seq task, where the latest GPT4 checkpoint still has a 23\% error rate (see Section \ref{aba1} for details). Thus, considering the deployment cost and the future potential of adding more features, we fine-tuned a local LLM with an augmented dataset consisting both input queries and output JSONs.

\subsubsection{Construct Causal-Retrieval-Bench} \label{Step1:data}
% reasoning
To the best of our knowledge, the aforementioned customized input-output pairs can not be collected from the online corpus, since the commonly used LLM training data are mainly conversational materials other than structured data.  
Therefore, we choose to construct a customized corpus containing both synthetic causal questions and the corresponding JSON representations by prompting an instruction-following LLM.

To collect LLM-generated data, the common approach starts from writing several demonstrated examples. Those demonstrations are then fed to an LLM (e.g., GPT-4) for paraphrasing. We have observed that such an approach suffers from (1) non-controllable topics and variables of interest, which results in content homogeneity, (2) incomplete/non-compliant JSON outputs, and (3) inappropriate paraphrase, where the causal question is transformed to be association-related. To resolve the pain points and prevent data contamination, we propose a three-course procedure, which is illustrated in Figure \ref{fig:retrieval-bench-ill}.

\input{Tables/Figure3}

% details
The procedure can be summarized as an output-first strategy, where the major goal is to improve the correctness and the variety of the output JSON first. An instruction prompt is incorporated to construct causal-related questions in different sentence structures. Specifically, we conducted value generation to prepare a topic database, JSON generation by sampling, and question paraphrasing with prompting. 
\begin{itemize}
    \item \textbf{Value Generation}: the goal of the first course is to get a candidate pool of the interested topic and variables similar to the RapidAPI\footnote{https://rapidapi.com/hub} hierarchy tree. We prompt the GPT model to generate some potential topics and related variable names. For each variable, we perform a zero-shot classification by GPT to determine the variable class, i.e., whether it is discrete or continuous. All the collected information is maintained in a three-level hierarchy structure (topic -> variable -> class).
    \item \textbf{JSON Generation}: Based on the assumption that causality tasks often involve variables within the same topic, we randomly generate structured JSON data following the topic-variable-class structure. For example, for an average treatment effect estimation task, a topic name is firstly drawn from the stem of the tree as the data file name, and two variables underneath are then considered as candidates for the synthetic treatment and outcome. For causal tasks where a specific group variable is needed, we sampled a random value, either continuous or discrete, based on its class.
    \item \textbf{Question Generation}: For each JSON output, we prompt the GPT model to generate five related questions given the context. Utilizing a univariate prompt template, we transform each JSON into an information-augmented prompt consisting of task-specific descriptions, expert-written demo examples, JSON information, and paraphrasing restrictions.
%prompt
Specifically, we implement GPT prompts in this step by a modulized template to improve components' reusability. Structurally speaking, the prompt starts with a description of the question generation task and the corresponding causal task. It is then followed by information extracted from a JSON from the previous course as the contextual component for the generated question. Subsequently, randomly sampled demonstrations are included as the sample illustrations and output restrictions are itemized as the final remark. 
\end{itemize}

During development, the aforementioned three courses are executed sequentially with quality control on the correctness of generated entities/queries in between. Confused with other statistical concepts, such as correlation and association, the current ChatGPT model has suboptimal performance on the causality-related task.  Hence, domain experts are involved after each step to improve the data quality with human annotation. As a result, for the Causal-Retrieval-Bench, we collect 1,500 pairs, i.e., 300 for each causal task, of causal questions with the corresponding JSON outputs.

\subsubsection{Fine-tuning a Large Language Model}
%\textcolor{red}{!TODO: move all the notations to this section}
%connect
After collecting a custom dataset containing causal questions and interpreted intents in a structured format, 
%intro
we fine-tune the LLaMA 2 pre-trained model checkpoints for learning underlying language patterns. 
%notation
We denote the input-output pairs as $\mathcal{D} = \{q_i, j_i\}$ for $i = 1, 2, ..., N$, where both inputs $q_i$ and outputs $j_i = \{c_i,\mathcal{V}_i\}$ can be separated and padded into word tokens $q_i = [q_{i1}, q_{i2},..., q_{iM}]$ and $j_i = [j_{i1}, j_{i2},..., j_{iL}]$ with length $M$ and $L$ respectively. 
%language modeling
A language model checkpoint is denoted as $\mathbb{G}$ which takes the language sequence as input and returns the word probability distribution $P(\cdot)$ for each word for each position with a total length of $L$. 
The possible input-output word token is limited in a finite dictionary $\mathbb{V} = \{w_1, w_2, ..., w_V\}$ with a cardinal of $V$.
We optimize the causal language modeling loss $\ell$, a cross-entropy loss on the token level, with $S$ sample of augmented dataset $\mathcal{S}' \subset \mathcal{S}$ as follows:
\begin{eqnarray}
\ell(\mathbb{G}, \mathcal{S}') 
& = & \frac{1}{S'} \sum_{i=1}^{S'} \ell(\mathbb{G}(q_i), j_i) \nonumber \\
& = & \frac{1}{S'L} \sum_{i=1}^{S'} \sum_{k=1}^L \textrm{cross-entropy} (\mathbb{G}(q_i)_k, j_{ik}) \nonumber \\
& = & \frac{1}{S'L} \sum_{i=1}^{S'} \sum_{k=1}^L \sum_{l=1}^V -I(j_{ik} = w_l) log(P(\mathbb{G}(q_i)_k) = w_l),  \nonumber
\end{eqnarray}
where the $\mathbb{G}(q_i)_k = t_k$ denotes the output word probability distribution at the $k$-th position, and the cross-entropy loss for that position can be calculated by the logarithm of the probability of word token $j_{ik}$. Minimizing such loss function can encourage the probabilistic model $\mathbb{G}$ to generate similar output to $j_i$ when given an input of $q_i$.

%LoRA
We implement the Low-Rank Adaptation (LoRA) \citep{lora} for parameter-efficient fine-tuning since the pre-trained checkpoint has more than $7$ billion parameters and it is computationally inefficient. Instead of changing all parameters in the model, LoRA only tunes adapters' weight and fixes the entire pre-trained checkpoint. Empirical study shows a relatively small number of ranks like $16$ perform very well in our use case.


==> 3_2_STEP2.tex <==

\subsection{STEP2. Assign and Execute Causal Tools}\label{sec:step2}
In this stage, to address user queries, we first select suitable causal learning algorithms based on the task class determined in Step 1, as depicted in Figure \ref{fig:step2}. Following this selection, the algorithm is executed automatically, using both the extracted information from Step 1 and the user-provided dataset as inputs, to get the estimated result. Depending on the causal task, the output result can be a causal graph $\mathcal{G}$, numerical values of estimated causal effect (estimated expected value of $\mathcal{Y}$), or a treatment level $a\in \mathcal{A}$. LLM4Causal facilitates a variety of approaches for each causal task by leveraging well-known public causal packages, including econml\citep{oprescueconml}, causalml\citep{chen2020causalml}, causal-learn\citep{zheng2023causal}, and CausalDM\citep{CDM}. Additionally, we remark that LLM4Causal is designed with flexibility, allowing for the incorporation of new methodologies through the simple integration of function scripts. In the current version, LLM4Causal randomly selects a method for analysis. However, we are in the process of enhancing LLM4Causal for a subsequent release, which aims to provide i) a more interactive platform where users can specify their preferred methods; ii) a comprehensive causal analysis report, offering outputs from all methods with detailed comparisons upon request; and iii) an advanced method selection feature for automatically determining the most suitable approach.

\begin{figure}
    \centering
    \includegraphics[width = \textwidth]{Fig/LLM4Causal-Step2.png}
    \caption{Causal Tool Assignment and Execution in the Second Step}
    \label{fig:step2}
\end{figure}


==> 3_3_STEP3.tex <==
\subsection{STEP3. Interpret the Numerical Output}\label{sec:step3}
%background
As discussed in Section \ref{sec:step2}, Step 2 produces a numerical value of causal effect, a recommended action level, or an adjacency matrix indicating causal relations in a causal graph.
% The function call produces either a set of numbers or an adjacency matrix that indicates the causal relationships. 
Interpreting these outputs needs domain expertise and may not be easily understood by a general audience lacking a causal background.
%intro
To enhance user-friendliness and reduce the learning curve of LLM4Causal, our final stage entails the interpretation of the function output using fluent natural language. The process starts with a template interpretation that automatically converts the numerical output to a one-sentence summary (See Appendix \ref{Step3:template} for examples). The final human-readable interpretation is then produced through the utilization of a calibrated LLM, which is guided by a designed prompt and uses the template summary and other information as input. The prompt instructs the LLM to avoid generating hallucinatory content, ensure the inclusion of all relevant information, and provide cohesive responses in the relevant context of the original question (See Appendix \ref{Step3:Prompt} for details).

Admittedly, we may directly take the crafted prompt and let a pre-trained LLM such as GPT-4 generate interpretation for us. However, the interpretations obtained this way are problematic. Human annotations indicate that about 25\% of the outputs exhibit hallucinations, 10\% contain missing information, and 35\% lack fluency (see their definition below).
%and further comparisons in Section \ref{aba2}
 Therefore, we calibrated the LLM model with additional human annotated interpretations for more accurate  interpretation results and
the prompt includes the aforementioned entities as basic elements and a graphical illustration can be found in Figure \ref{fig:interpret-bench-ill}.  

In the following, we outline the process used to generate the golden dataset Causal-Interpret-Bench. The approach for model fine-tuning is similar to that used in step 1 and is omitted here for brevity.

\input{Tables/Figure5}

\subsubsection{Build Causal-Interpret-Bench} \label{sec33}
Likewise to the procedures in Step 1, we first use the GPT model to generate a silver dataset of interpretations, employing the templates in Appendix \ref{Step3:template} and the prompts in Appendix \ref{Step3:Prompt}. Among the required inputs, user queries and their corresponding causal task classifications from section \ref{Step1:data} are reused. Using the methodology described in \ref{sec:step2}, we paired the existing information with a causal function. As for the function outputs, the numerical values
% /graph results 
are randomly generated in formats specific to each task. To create the final golden dataset, we then have annotators manually revise 400 interpretations, adhering to the evaluation rubric outlined below:
\begin{itemize}
    \item \textbf{Hallucination}: i) The interpretation incorrectly presents information, such as treating the response variable as the treatment variable and misinterpreting the direct effect in mediation analysis as the total effect; ii) it includes details that are not present in the provided context, such as commenting on the effectiveness of methods used; or iii) it incorrectly applies terms such as `correlation' and `association', which are inappropriate for describing causal relations.
    
    \item \textbf{Incompleteness}: The interpretation lacks one or more essential components, such as the data set, the method, the results, and / or all the variables involved.
    
    \item \textbf{Non-fluency}: i) The interpretation includes unexplained, meaningless variable names (e.g., 'chg\_rate'); ii) it repeats the same content multiple times; or iii) it directly references or rephrases the guidelines in the prompt.
\end{itemize}

Although various metrics are developed to assess the factual consistency between output summaries / interpretations and the original context \cite{zhang2019bertscore} or to assess the conciseness and readability of output summaries, such as the ROUGE score \cite{lin2004rouge}, they are not representative of our specific needs. The interpretation we require is highly specialized, necessitating a clear distinction between causality and association, guaranteeing that no crucial information is missed, and ensuring it is comprehensible to general audiences, among other requirements. 
The current automatic evaluation based on sentence similarity metrics fails to adequately incorporate human preferences, making them unsuitable for our application. Therefore, instead we carefully defined the three aforementioned rubrics to guide human annotation.

==> 4_2_Benchmark_models.tex <==
\subsection{Benchmark models}
The Large language models for evaluation are described as follows.
\begin{itemize}
    %\item \textbf{gpt3.5-turbo} \citep{GPT3}: 
    \item \textbf{gpt4-turbo} \citep{openai2023gpt4}: GPT4 with the function call feature enabled. By creating a function with causal task description and input arguments requirements, we utilize the GPT 4 with the function calling feature to generate the output, which is then transformed into JSON format based on the predicted "causal\_problem" key. 
    \item \textbf{LLM4Causal-Retrieve}: A customized language model started from Llama-2 (7B) checkpoint and further fine-tuned\footnote{with 10\% held out for validation purpose. The same setting applies to the Causal-Interpret-Bench} on the Causal-Retrieval-Bench.  
    \item \textbf{LLM4Causal-Interpret}: We provided Causal-Interpret-Bench as extra instructions to the Llama-2 (7B) checkpoint.
    \item \textbf{LLM4Causal-Mixed}: The same setting as the previous two models, but with a combination of both data sets.
\end{itemize}


==> 4_3_Main_Result.tex <==

\subsection{Main Result: End-to-End Evaluation} \label{e2e_exp}
In this experiment, we evaluate the end-to-end model performance starting from causal-related questions and resulting in interpretations explaining the function outputs. 

%We followed the same procedure of section \ref{Sec:proposed_method} and collected 150 additional questions with unseen topics and variables of interest. The purpose is to mask the signals from familiar topics that may provide unwanted advantages for our models. The datasets mentioned in each question are simulated per the procedure described in \ref{data_gen}. 

With such a setup, there is no sole "golden label" existing for each question as the correct interpretation is not unique. To provide a comprehensive analysis, we provide the following evaluation metrics inspired by previous works \citep{gpt4tools} and \citep{toolllm} from two aspects:
\begin{itemize}
    \item \textbf{Pass rate} \citep{toolllm}: it calculates the proportion of user requests that could be completed by the model. This metric measures the model's executability, which is a fundamental requirement for the LLM model. It could be calculated as $\text{Pass rate}=\frac{1}{N}\sum_{i=1}^{N}\mathbb{I}\{\tau_i\}$, where $N$ is the number of samples, $\mathbb{I}\{\tau_i\}$ is an indicator function, which equals to 1 if the model could generate an output for the $i^{th}$ user request, and 0 otherwise.
    \item \textbf{Relevance rate}: it calculates the proportion of user requests that the model provides a relevant output which is about the correct causal task. This metric measures the model's task identification ability, which directly affects the model's feasibility in executing appropriate causal functions. It could be calculated as $\text{Relevance rate}=\frac{1}{N}\sum_{i=1}^{N}\mathbb{I}\{\gamma_i\}$, where $N$ is the number of samples, $\mathbb{I}\{\gamma_i\}$ is an indicator function, which equals to 1 if the model could generate an output that correctly the causal task for the $i^{th}$ user request, and 0 otherwise.
    \item \textbf{Win rate}: it calculates the proportion of user requests that the model has delivered an accurate result. This metric measures the model's accuracy, which is essential to lift users' experience. It could be calculated as $\text{Win rate}=\frac{1}{N}\sum_{i=1}^{N}\mathbb{I}\{\eta_i\}$, where $N$ is the number of samples, $\mathbb{I}\{\eta_i\}$ is an indicator function which equals to 1 if the model output contains the desired true value for the $i^{th}$ user request, and 0 otherwise.
    %\footnote{Specifically, for ATE, HTE, CGL and MA, the results are considered as accurate if the estimated causal graph or causal effects are close to the true value. For OPO, the resulted policy is considered to be accurate if the actions recommended always bring to the highest cumulative rewards.} 
    % it consistently outperforms the random policy and greedy policy that only maximizes the observed rewards(compare optimal action rather than value instead).
\end{itemize}

To the best of our knowledge, there is no other implementation that can finish end-to-end causal-question answering, so we only evaluated performance metrics for LLM4Causal-Mixed in Table \ref{table:main}.

\begin{table}[H]
\centering
\caption{End-to-end evaluation for LLM4Causal-Mixed}
\begin{tabular}{rlllll}
\hline
               & CGL  & ATE  & HTE  & MA   & OPO  \\ \hline
Pass Rate      & 1.00 & 0.93 & 0.83 & 0.86 & 0.83 \\
Relevance Rate & 1.00 & 0.93 & 0.83 & 0.80 & 0.83 \\
Win Rate       & 0.90 & 0.90 & 0.80 & 0.70 & 0.73 \\ \hline
\end{tabular}
\label{table:main}
\end{table}

%MORE DISCUSSION
The relevance rate measures the interpretation w.r.t. causal task relevancy, and we can see that from the testing set our model works quite well, which only made 2 mistakes in the mediation analysis and viewed them as average treatment effect problems incorrectly. As for the win rate, we have $90\%$ performance on both causal graph learning problem\footnote{evaluated based on ground truth and outputs manually} and average treatment effect. The heterogeneous treatment effect questions and off-policy optimization problems are similar in input-output patterns and our model has similar performances%, and a part of (XX\%) errors are the result of mismatching data columns by interpreting the user question. 
Finally, the performance of the mediation analysis is sub-optimal, we found that it is mainly because the model may miss one of three numerical results even though the mediation function is called correctly (please see more details from Section \ref{aba2}).


==> 4_4_AblationAnalysis1.tex <==

\subsection{Ablation Analysis 1: Causal Entity Extraction} \label{aba1}
In this section, we focus the model performance on Step 1, user request interpretation, comparing with the benchmark methods on the synthetic data of 150 topics. In detail, for each simulated user request, the model is asked to produce a JSON output following the output format listed in Table \ref{tab:input-output-example}. The accuracy of each key value is then calculated by comparing the ground true label with the model outputs, for each key value. It is worth mentioning that, we require an exact match for causal task and data set values since the causal task lists are provided in the training data and the dataset names are explicitly mentioned in the user request. For the other key values, we consider the value correct if the major component for the variable name is covered in the model output. 

We used the GPT4 with the function call feature enabled. It was developed by OpenAI in 2023 and demonstrated a strong capability of zero-shot function selection and argument extraction. Multiple papers \citep{toolllm, graphtoolformer} treated its output as the golden label for local LLM development.

% and the output was validated by the ground truth label by comparing the value for each key. The accuracy scores for correctly specifying the causal task classification and exactly matching the values under each key are reported. As a consequence of different causal tasks having variant keys, if the model misclassifies the causal task in the first place, its performance for the corresponding keys to the problem will be harmed.
% Here we are reusing the annotated $150$ samples with unseen topics from the training data and focusing on step 1. 

% Here we are benchmarking GPT4 with the function call feature enabled. It was developed by OpenAI in 2023 and demonstrated a strong capability of zero-shot function selection and argument extraction. Multiple papers \citep{toolllm, graphtoolformer} treated its output as the golden label for local LLM development. We created one function with detailed descriptions for each causal task with the specification of required input arguments, the output was mapped into one JSON with an additional "causal\_problem" key storing the selected function. 

%\begin{table}[H]
%\caption{Causal Entity Extraction Performance (Previous)}
%\centering
%\begin{tabular}{lccccccc}
%\hline
%                      & Causal Task & Dataset & Nodes & Treatment & Response & Mediator & Condition \\ \hline
%gpt3.5-turbo          &  0.77 &  0.77 & 0.27 & 0.60 & 0.61 & 0.81 & 0.33\\
%gpt3.5-turbo (guided) & - & 1.00 & 0.27 & 0.84 & 0.80 & 0.94 & 0.42 \\ 
%gpt4-turbo            & 0.77           & 0.77    & 0.27  & 0.67      & 0.62     & 0.67     & 0.32      \\ 
%gpt4-turbo (guided)   & -              & 1.00    & 0.27  & 0.90      & 0.86     & 0.97     & 0.40      \\ \hline
%LLM4Causal-Retrieve   & 0.98           & 0.95    & 0.81  & 0.97      & 0.98     & 0.94     & 0.97      \\
%LLM4Causal-Mixed      & 0.99           & 0.99    & 0.88  & 0.98      & 0.97     & 1.00     & 0.98      \\ \hline
%\end{tabular}
%\label{tab:step1-bench}
%\end{table}


\begin{table}[H]
\caption{Causal Entity Extraction Performance}
\centering
\begin{adjustbox}{width=0.95\columnwidth,center}
\begin{tabular}{lccccccc}
\hline
                      & Causal Task & Dataset & Nodes & Treatment & Response & Mediator & Condition \\ \hline
gpt4-turbo            & 0.69(0.02)  & 0.99(0.01)  & 0.99(0.02)  & 0.60(0.02) & 0.60(0.02) & 0.61(0.04) & 0.98(0.01) \\ \hline
LLM4Causal-Retrieve      & 0.96(0.00\footnote{less than 0.01})  & 0.99 (0.01)    &  0.88(0.03)  & 0.94(0.00)  & 0.94(0.01)     & 0.90(0.05)    & 1.00(0.01)      \\
LLM4Causal-Mixed      & 0.98(0.00)      & 1.00(0.00)    & 1.00(0.00)  & 0.96(0.00)   & 0.97(0.00)     & 1.00(0.00)    & 1.00(0.00)      \\ \hline
\end{tabular}
\end{adjustbox}
\label{tab:step1-bench}
\end{table}

As shown in the table \ref{tab:step1-bench},  we can see that both LLM4Causal models can solve the seq2seq problem very well and significantly outperform GPT-based models. This is driven by the accuracy of the causal task identification, which blocks the model from accurately finding necessary entities to extract if a wrong causal model is posited. Besides, a seemingly surprising fact is the mixed version even outperforms the retrieve-only version on every task. Such a phenomenon may be due to the inclusion of the interpretation data, which also involves causal queries and their corresponding causal tasks with interpretations, increasing the parameter weight during the fine-tuning process of the model between causal tasks and their meanings.

%Meanwhile, we can find out that the turbo version of both GPT3.5 and GPT4 is doing well on some function argument extraction tasks, but their accuracy in identifying the correct causal task is limited. To compare the model performance solely on each causal entity, we provide GPT-based models with additional inputs by only feeding the correct function to the model (marked as guided) and try to investigate if the performance was masked by selecting the incorrect causal task. 

%It is shown in the table \ref{tab:step1-bench} that the turbo version of both GPT3.5 and GPT4 can perform the causal task identification task relatively well, but their accuracy on detailed argument extraction is limited, especially for keys with complicated formats such as condition and nodes. As a further step, we only provided the correct function to the model (marked as guided) and tried to investigate if the performance was masked by selecting the incorrect causal task. We can see significant improvement as expected. For gpt4 specifically, we had an increase in the dataset ($0.77 \rightarrow 1.00$), treatment ($0.67 \rightarrow 0.90$), response ($0.62 \rightarrow 0.86$), and mediator ($0.67 \rightarrow 0.97$), but it still made considerable mistakes on exactly matching nodes and conditions. As for LLM4Causal, we can see that both checkpoints can solve such a seq2seq problem very well, only the Condition key having an exact match accuracy rate that is less than $0.9$. A seemingly surprising fact is the mixed version even outperforms the retrieve-only version on most tasks except the nodes, which may be due to the inclusion of the interpretation data, which also involves causal queries and their corresponding causal tasks with interpretations, increasing the word connection between causal tasks and their meanings.


==> 4_5_AblationAnalysis2.tex <==

\subsection{Ablation Analysis 2: Interpreting Causal Function Output} \label{aba2}
Following metrics described in section \ref{sec33}, we evaluate the quality of model-generated interpretations from multiple sources. A double-blind experiment is conducted with domain experts judging if the interpretation generated by a language model has an issue with hallucination, fluency, or incompleteness. The averaged error rate is reported in Table \ref{tab:step3-bench}.

\begin{table}[H]
\caption{Causal Result Interpretation Performance, where hall. indicates hallucination, inco. stands for incompleteness, and fluent is for non-fluency}
\centering
\label{tab:step3-bench}
\begin{tabular}{rrcccrccc}
\hline
model                &    task   &  hall. & inco. & fluent & task   &  hall. & inco. & fluent \\ \hline
 gpt4-turbo           &\multirow{3}{*}{CGL} & 0.08          & \textbf{0.00}       & 0.28  & \multirow{3}{*}{MA}         & \textbf{0.05}          & \textbf{0.10}       & 0.22       \\
 LLM4Causal-Interpret &                     & \textbf{0.05}          & 0.03       & 0.28    &                  & 0.10          & 0.15       & 0.18         \\
LLM4Causal-Mixed     &                     &  0.23          & \textbf{0.00}       & \textbf{0.20}    &                        & 0.19          & 0.27       & \textbf{0.16}        \\ \hline
gpt4-turbo           & \multirow{3}{*}{ATE} &  0.43          & 0.05       & 0.48    & \multirow{3}{*}{OPO}     & \textbf{0.15}          & \textbf{0.10}       & 0.33    \\
LLM4Causal-Interpret &                     &  0.38          & 0.10       & \textbf{0.20}     &                     & 0.26          & 0.13       & 0.18       \\
LLM4Causal-Mixed     &                     &  \textbf{0.28}          & \textbf{0.00}       & 0.50     &                        & 0.21          & 0.13       & \textbf{0.10}      \\ \hline
gpt4-turbo           &\multirow{3}{*}{HTE} &  0.08          & \textbf{0.00}       & 0.28    & \multirow{3}{*}{\textbf{All}}          & 0.19          & \textbf{0.06}       & 0.36         \\
LLM4Causal-Interpret &                     &  \textbf{0.05}          & 0.03       & 0.28     &            & \textbf{0.17}          & 0.10       & \textbf{0.20}       \\
LLM4Causal-Mixed     &                     &  0.23          & \textbf{0.00}       & \textbf{0.20}   &         & 0.20          & 0.08       & 0.28        \\ \hline
\end{tabular}
\end{table}

\begin{comment}
\begin{table}
\caption{Causal Result Interpretation Performance}
\centering
\label{tab:step3-bench}
\begin{tabular}{rrccc}
\hline
                     & model                & hallucination & incomplete & non-fluent \\ \hline
\multirow{3}{*}{CGL} & gpt4-turbo           & 0.08          & \textbf{0.00}       & 0.28       \\
                     & LLM4Causal-Interpret & \textbf{0.05}          & 0.03       & 0.28       \\
                     & LLM4Causal-Mixed     & 0.23          & \textbf{0.00}       & \textbf{0.20}       \\ \hline
\multirow{3}{*}{ATE} & gpt4-turbo           & 0.43          & 0.05       & 0.48       \\
                     & LLM4Causal-Interpret & 0.38          & 0.10       & \textbf{0.20}       \\
                     & LLM4Causal-Mixed     & \textbf{0.28}          & \textbf{0.00}       & 0.50       \\ \hline
\multirow{3}{*}{HTE} & gpt4-turbo           & 0.08          & \textbf{0.00}       & 0.28       \\
                     & LLM4Causal-Interpret & \textbf{0.05}          & 0.03       & 0.28       \\
                     & LLM4Causal-Mixed     & 0.23          & \textbf{0.00}       & \textbf{0.20}       \\ \hline
\multirow{3}{*}{MA}  & gpt4-turbo           & \textbf{0.05}          & \textbf{0.10}       & 0.22       \\
                     & LLM4Causal-Interpret & 0.10          & 0.15       & 0.18       \\
                     & LLM4Causal-Mixed     & 0.19          & 0.27       & \textbf{0.16}       \\ \hline
\multirow{3}{*}{OPO} & gpt4-turbo           & \textbf{0.15}          & \textbf{0.10}       & 0.33       \\
                     & LLM4Causal-Interpret & 0.26          & 0.13       & 0.18       \\
                     & LLM4Causal-Mixed     & 0.21          & 0.13       & \textbf{0.10}       \\ \hline
\multirow{3}{*}{\textbf{All}} & gpt4-turbo           & 0.19          & \textbf{0.06}       & 0.36      \\
                     & LLM4Causal-Interpret & \textbf{0.17}          & 0.10       & \textbf{0.20}       \\
                     & LLM4Causal-Mixed     & 0.20          & 0.08       & 0.28       \\ \hline
\end{tabular}
\end{table}
\end{comment}

Regarding LLM4Causal Performances, we can see that the Interpret checkpoints are comparable to or superior to the GPT-4-turbo's performance on both hallucination and fluency metrics, indicating that a model fine-tuning can reduce domain-related hallucination, e.g. "association" vs "causality" in this study, and make the interpretation crisp without including sentences repeating already-stated information. Besides, we can see that our fine-tuned models still have space to improve, especially in including all necessary components for the mediation analysis, which is the reason for an inferior score on the incompleteness. 

%From this study, even though the performance comparison between the LLM4Causal-Interpret and the LLM4Causal-Mixed has different winners on both hallucination ($0.17$ vs $0.20$) and incompleteness ($0.20$ vs $0.28$). Based on the available experiment, we are suggesting fine-tuning only one model with a mixture of data for the sake of computational efficiency but having more data points on the interpretation task, which may further improve the current performance.Z

==> Mis/backup.tex <==
%\subsection{End-to-End Performance Evaluation: A Case Study}
%The user experience of our work is demonstrated in figure \ref{fig:csl-demo}, \ref{fig:ate-demo}, and \ref{fig:hte-demo}, which presents the capabilities of answering causal-related questions with LLM4Causal as a chatbot. For each of the CGL, ATE, and HTE tasks, we show one end-to-end example. The demo website is developed by the Streamlit\footnote{https://streamlit.io/} package in Python with the intention that users can chat with our model as a ChatGPT-like environment with causal problem-solving ability. All three examples use a publicly available dataset called "cancer\_1000\_1.csv" from \cite{li2018bayesian}. %One causal-related question for the aforementioned tasks is written as a demonstration.

%\begin{figure}[H]
%    \centering
%    \includegraphics[width=10cm]{Fig/csl_v1.png}
%    \caption{Demo Example of Answering Causal Structure Learning Question}
%    \label{fig:csl-demo}
%\end{figure}

%Figure \ref{fig:csl-demo} shows the system results (including intermediate steps) for the question "What is the causal relationship between smoking and cancer in the cancer\_1000\_1.csv dataset?" and LLM4Causal successfully identified it as a CGL task with the JSON output "{'causal\_problem': ['CSL', 'CGL'], 'dataset': ['cancer\_1000\_1.csv'], 'covariates': [None]}". The screenshot does not capture them due to the web page limit. After the JSON step (step 1 in \ref{sec:step1}), the service loaded the data from the hard drive and triggered a PC algorithm to discover the causal relationship between the interested variables. Finally, the original questions were answered in natural language, using the results from the graph\_learning function.

%\begin{figure}[H]
%    \centering
%    \includegraphics[width=10cm]{Fig/ate_v1.png}
%    \caption{Demo Example of Answering Average Treatment Effect Question}
%    \label{fig:ate-demo}
%\end{figure}


%\begin{figure}[H]
%    \centering
%    \includegraphics[width=10cm]{Fig/hte_v1.png}
%    \caption{Demo Example of Answering Heterogeneous Treatment Effect Question}
%    \label{fig:hte-demo}
%\end{figure}

%Both figure \ref{fig:ate-demo} and figure \ref{fig:hte-demo} showcase the full conversation between the user and LLM4Causal. The difference between these two examples is if we wanted the effect estimation limited to a specific group of populations. If so (for example pollution = "high") then we need to trigger the heterogeneous treatment effect instead of the average treatment effect with an additional input "condition". We can see that LLM4Causal discriminated different problems prosperously and provided reasonable interpretations based on the provided context.

%\subsection{Ablation Analysis}
%We also carefully evaluated the model performance with an ablation analysis to determine the effectiveness of % each step/sub-module with a focus on 
%the causal entity extraction described in section \ref{sec:step1}. %Secondly, we compared the interpretation ability using the metrics depicted in the section \ref{sec33}. For both studies, o
%Our fine-tuned model is benchmarked with a GPT4 variant (with or without function call features). As a further step, more simulation studies involving end-to-end and interpretation evaluation will be released soon.

%As for LLM4Causal, we trained %three 
%two different checkpoints: `LLM4Causal-Retrieve' only trains on Causal-Retrieval-Bench%, `LLM4Causal-Step3` has access to Causal-Interpret-Bench, 
%and `LLM4Causal-Mixed' or `LLM4Causal' simultaneously trained on both datasets. The purpose of showcasing `LLM4Causal-Mixed' and `LLM4Causal-Retrieve' is to show that mixing both sources of the augmented data will not harm the inference quality and that only having one univariate model is sufficient. 

==> Mis/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Tables/Figure3_App.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[height = 4cm]{Fig/step1_v4.png}
    \caption{Causal-Retrieval-Bench construction procedures for the first step. GPT prompts used in this section can be found in Appendix \ref{ch3:step1}. In the left panel, GPT is prompted to list out different topics and measurable variables for each topic. With randomly drawn tasks from section \ref{Sec:problem_formulation} and some variables under the same topic, we generated JSON output in the middle panel. The colored boxes in the left and middle panels are shared topics and variable names of interests. In the right panel, the numbered boxes in template 2 mean blank places to be filled with the task description, the supplied demonstration, JSON inputs, and output restrictions. Common connectors and general instruction in prompt 2 are shortened into "xxxxx" due to the figure limit.}
    \label{fig:retrieval-bench-ill}
\end{figure}

==> Tables/Table2_App.tex <==
\begin{table}[H]
\centering
\caption{Example Query Inputs with expected JSON Outputs}
\vspace{2pt}
\label{tab:input-output-example}
\begin{tabular}{lp{2.5in}p{2.5in}}
\hline
Task  & Example Input Query                                                                                                                                                                                                                                   & Expected JSON Output                                                                                                                                                                                                       \\[0.05cm] \hline
CGL & Does the disaster\_risk\_reduction.csv dataset provide evidence of a direct link between building code compliance rate and the effectiveness of disaster preparedness campaigns?                                                                      & \{'causal\_problem': {[}'CSL', 'CGL'{]}, 'dataset': {[}'disaster\_risk\_reduction.csv'{]}, 'nodes': {[}'building\_code\_compliance\_rate', 'disaster\_preparedness\_campaigns'{]}\}                                         \\[0.2cm]
ATE & How does the labor force participation rate (labor\_participation\_rate) in employment.csv contribute to changes in wage growth (wage\_increase)?                                                                                                     & \{'causal\_problem': {[}'CEL', 'ATE'{]}, 'dataset': {[}'employment.csv'{]}, 'treatment': {[}'labor\_participation\_rate'{]}, 'response': {[}'wage\_increase'{]}\}                                                          \\[0.2cm]
HTE & Based on the findings in the cybersecurity.csv dataset, what impact does the presence of data breach incidents have on cybersecurity investment under a group condition where the cybersecurity readiness index is set at 0.5 (readiness\_index=0.5)? & \{'causal\_problem': {[}'CEL', 'HTE'{]}, 'dataset': {[}'cybersecurity.csv'{]}, 'treatment': {[}'data\_breach\_incidents'{]}, 'response': {[}'cybersecurity\_investment'{]}, 'condition': {[}('readiness\_index', 0.5){]}\} \\[0.5cm]
MA  & Is there substantial evidence in retail.csv indicating that the pathway from retail employment to the e-commerce penetration rate is mediated by the consumer confidence index?                                                                       & \{'causal\_problem': {[}'CEL', 'MA'{]}, 'dataset': {[}'retail.csv'{]}, 'treatment': {[}'retail\_employment'{]}, 'response': {[}'e-commerce\_penetration\_rate'{]}, 'mediator': {[}'consumer\_confidence\_index'{]}\}       \\[0.2cm]
OPO & If the poverty rate stands at 0.32 (poverty\_ratio = 0.32), what recommendations can be derived from the poverty.csv dataset on adjusting social assistance coverage to positively impact the gini coefficient?                                       & \{'causal\_problem': {[}'CPL', 'OPO'{]}, 'dataset': {[}'poverty.csv'{]}, 'treatment': {[}'social\_assistance\_coverage'{]}, 'response': {[}'gini\_coefficient'{]}, 'condition': {[}('poverty\_ratio', '0.32'){]}\}          \\[0.1cm] \hline
\end{tabular}
\end{table}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

